Compiler Support for Speculation in Decoupled Access/Execute Architectures

Irregular codes are bottlenecked by memory and communication latency. Decoupled access/execute (DAE) is a common technique to tackle this problem. It relies on the compiler to separate memory address generation from the rest of the program, however, such a separation is not always possible due to control and data dependencies between the access and execute slices, resulting in a loss of decoupling. In this paper, we present compiler support for speculation in DAE architectures that preserves decoupling in the face of control dependencies. We speculate memory requests in the access slice and poison mis-speculations in the execute slice without the need for replays or synchronization. Our transformation works on arbitrary, reducible control flow and is proven to preserve sequential consistency. We show that our approach applies to a wide range of architectural work on CPU/GPU prefetchers, CGRAs, and accelerators, enabling DAE on a wider range of codes than before.

==> Figures/FigHoistingCFG.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.475\textwidth]{Figures/HoistingCFG.pdf}

 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/HoistingCFG_a.pdf}
 %     \caption{Original CFG. Pre-order of requests: $b, d, e, g$.}
 %     \label{fig:HoistingCFG_a}
 % \end{subfigure}%
 % \hfill%
 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/HoistingCFG_b.pdf}
 %     \caption{First iteration of hoisting. Pre-order of requests: $b, e, g, d$.}
 %     \label{fig:HoistingCFG_b}
 % \end{subfigure}%
 % \hfill%
 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/HoistingCFG_c.pdf}
 %     \caption{Second and last iteration of hoisting. Pre-order of requests: $b, e, g, d$.}
 %     \label{fig:HoistingCFG_c}
 % \end{subfigure}
 
 
\caption{An example of applying our iterative control-flow hoisting algorithm to enable speculative memory requests.}
\label{fig:HoistingCFG}
\end{figure}


==> Figures/FigMemoryAccessUnit.tex <==
\begin{figure}[t]
\centering
 % \begin{subfigure}[b]{0.45\textwidth}
     \centering
     \includegraphics[width=0.49\textwidth]{Figures/MemoryAccessUnit.pdf}
     % \caption{An architecture with decoupled address generation, memory access, and compute.}
     % \label{fig:MemoryAccessUnit_a}
 % \end{subfigure}
 % \hfill
 % \begin{subfigure}[b]{0.45\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/MemoryAccessUnit_stval.pdf}
 %     \caption{Loss-of-decoupling between address generation and memory access due to a dependency on the memory value.}
 %     \label{fig:MemoryAccessUnit_b}
 % \end{subfigure}

\caption{Organization of a typical data unit (DU) in a decoupled access/execute accelerator. Loads can execute out-of-order w.r.t. stores and are checked for read-after write (RAW) hazards. Store values are tagged with a poison bit that is used to drop corresponding mis-speculated store requests.}
\label{fig:MemoryAccessUnit}
\end{figure}


==> Figures/FigPhiChange.tex <==
\begin{figure}[t]
\centering

 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/PhiChange_a.pdf}
 %     \caption{}
 %     \label{fig:PhiChange_a}
 % \end{subfigure}
 % \hvill
 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/PhiChange_b.pdf}
 %     \caption{}
 %     \label{fig:PhiChange_b}
 % \end{subfigure}
 %  \hvill
 % \begin{subfigure}[b]{0.15\textwidth}
 %     \centering
 %     \includegraphics[width=\textwidth]{Figures/PhiChange_c.pdf}
 %     \caption{}
 %     \label{fig:PhiChange_c}
 % \end{subfigure}
 
 
\includegraphics[width=0.475\textwidth]{Figures/PhiChange.pdf}
\caption{The hoisting of \texttt{load consume} calls in the CU requires changing $\phi$-nodes to select instructions.}
\label{fig:PhiChange}
\end{figure}


==> Figures/FigTikzCFGs.tex <==

% \begin{center}
% \begin{tikzpicture}[auto,
%   node distance = 5mm,
%   start chain = going right,
%   box/.style = {draw,circle,blur shadow,fill=white,
%         on chain,align=center}]
%  \node[box] (b1)    {$x_1\leftarrow0$\\ $y_1\leftarrow0$};      
%  \node[box] (b2)    {$x_2\leftarrow\phi(x_1,x_3)$\\
%  $y_2\leftarrow\phi(y_1,y_3)$\\
%  $(x_2<10)$?};      
%  \node[box] (b3)    {$y_3\leftarrow y_2+x_2$\\ $x_3\leftarrow x_2+1$};  
%  \node[box] (b4)    {print($y_2$)};     
%  \begin{scope}[rounded corners,-latex]
%   \path (b2.-40) edge[bend left=50] (b4.40)
%   (b1) edge (b2) (b2) edge (b3);
%   \draw (b3.230) -- ++(0,-0.3) -| ([xshift=-5mm]b2.west) |-
%   ([yshift=3mm]b2.130) -- (b2.130);
%  \end{scope}
% \end{tikzpicture}
% \end{center}

\tikzstyle{midnode}=[
    draw=blue!70,   % draw the border with 70% transparent blue
    rectangle,      % the shape of the node is a rectangle
    fill=blue!10,   % fill the box with 20% blue
    text width=1cm,
    text centered]

\tikzstyle{smallnode}=[
    draw=blue!70,   % draw the border with 70% transparent blue
    rectangle,      % the shape of the node is a rectangle
    fill=blue!10,   % fill the box with 20% blue
    text width=0.4cm,
    text centered]

\begin{tikzpicture}[->,>=stealth,auto, very thick, scale=5]
        % Draw the vertices.
        \node[midnode] (s) {Start};
        \node[smallnode, right of=s, node distance=1.8cm] (a) {1};
        \node[smallnode, below of=a] (b) {2};
        \node[smallnode, right of=a, node distance=1.8cm] (c) {3};
        \node[smallnode, below of=c] (d) {4};
        \node[smallnode, right of=c, node distance=1.8cm] (e) {5};
        \node[midnode, below of=e] (x) {Stopp};

        % Connect vertices with edges
        \path (s) edge node {} (a);
        \path (a) edge node {} (c);
        \path (a) edge node {} (b);
        \path (b) edge node {} (c);
        \path (c) edge node {} (d);
        \path (c) edge node {} (e);
        \path (d) edge node {} (e);
        \path (e) edge node {} (x);

\end{tikzpicture}



